Observing the Invisible: Live Cache Inspection for High-Performance Embedded Systems

The vast majority of high-performance embedded systems implement multi-level CPU cache hierarchies. But the exact behavior of these CPU caches has historically been opaque to system designers. Absent expensive hardware debuggers, an understanding of cache makeup remains tenuous at best. This enduring opacity further obscures the complex interplay among applications and OS-level components, particularly as they compete for the allocation of cache resources. Notwithstanding the relegation of cache comprehension to proxies such as static cache analysis, performance counter-based profiling, and cache hierarchy simulations, the underpinnings of cache structure and evolution continue to elude software-centric solutions. In this paper, we explore a novel method of studying cache contents and their evolution via snapshotting. Our method complements extant approaches for cache profiling to better formulate, validate, and refine hypotheses on the behavior of modern caches. We leverage cache introspection interfaces provided by vendors to perform live cache inspections without the need for external hardware. We present CacheFlow, a proof-of-concept Linux kernel module which snapshots cache contents on an NVIDIA Tegra TX1 SoC (system on chip).

==> responses.tex <==
\section*{Revision Letter}
{%\setstretch{0.91}

We want to thank the reviewers for the insightful comments and the
opportunity to significantly improve our manuscript.
A summary of
the changes and answers to the concerns raised by the reviewers are
provided below.

%% Commenting this out, since this is already addressed at the end.
%% RM, feel free to uncomment if you disagree.
\subsection{Meta Review Comments}

\begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label={\bf MR\arabic*:}]
\item {\bf\emph{[...] The authors have to include new results as a
    proof/evidence that the tool can reveal a hard-to-find issue or to
    better answer a question regarding LLC performance.}}
  
  In our evaluation, we previously focused on the usage scenarios (1),
  (2), (3), and (4) mentioned in Section~\ref{sec:usage_scenarios}. In
  the revised manuscript, we have added four more
  experiments to reinforce two main points that were not
  well supported in the original draft: (A) that \cachedump can 
  derive metrics on cache usage based on the actual
  content of the snapshots. This cannot be done with
  performance counters-based analyses. The metric is capable of
  predicting clash on cache resources for co-running applications. It
  outperforms the typical WSS-based metric that can be constructed
  with performance counter-based analysis
  (Section~\ref{sec:ev_compat}). (B) That one can study the properties
  of the cache replacement policy. The latter point is demonstrated by
  confirming that the LLC indeed employs a random replacement policy;
  and by studying the probabilities that each way is selected for
  allocations (Section~\ref{sec:ev_repl}).

\item {\bf\emph{[...] This study lacks sufficient
    discussion/analysis of the instrumentation overhead.}}

  We distinguish between ``Flush'' and ``Transparent'' modes in
  Section~\ref{sec:overview}. The latter was not previously discussed
  because it was not used in the evaluation.  We have also added an
  evaluation of the overhead introduced by \cachedump in the main
  modes of operation in terms of both pollution of the cache and time
  required to acquire a snapshot. The evaluation is presented in
  Section~\ref{sec:ev_overh}. We have also removed the previous study
  that created some misunderstanding concerning overhead.
  
\item {\bf\emph{[...] In addition, a just comparison against a
    hardware-based approach (e.g., JTAG) is also necessary in terms of
    cost \$ and side effects.}}

  We have added a brief paragraph about the cost/benefit tradeoff of
  \cachedump compared to hardware debuggers. In a nutshell,
  inexpensive JTAG debuggers cannot be used out of the box to perform
  cache content analysis. It is actually an open research question
  whether this would be at all possible over the JTAG interface. At
  the time of this writing, the authors are aware of two debuggers
  that are capable of dumping CPU cache contents: (A) The ARM DS-5
  Debugger in combination with the
  DSTREAM\footnote{\url{https://store.developer.arm.com/store/debug-probes/dstream-st-debug-adapter}}
  adapter; (B) The Lauterbach Power Trace
  II\footnote{https://www.lauterbach.com/frames.html?cacheanalyzer.html}. Both
  are rather expensive ($>$ USD 6,000). Debuggers capable of
  performing cache content analysis exploit high-bandwidth trace
  ports. Also note that even the DS-5 debugger cannot always guarantee
  that the state of caches is not modified when debugging\footnote{See
    \url{https://static.docs.arm.com/100953/0529/debugger_user_guide_100953_0529_00_en.pdf},
    Note under Figure 6-5.}. With a price-tag of USD~0, no requirement
  for the target to expose a trace port, the capability to analyze the
  cache of remote systems, and with only \texttildelow 1\% pollution
  overhead in full transparent mode (see Section~\ref{sec:ev_overh}),
  there exists compelling evidence that \cachedump is a useful technique.

\end{enumerate}

\subsection{Reviewer \#1}

\begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label={\bf Q\arabic*:}]

\item {\bf\emph{The experimental results are straightforward and
    well-know, little insights into the potential of this tool; the
    presented benchmark plots look reasonable, neither the plots nor
    the tool as it is described can unearth any new information about
    the behavior of the cache.}}

A: Although interpretable, the results in Section~\ref{sec:ev_sys} are
far from straightforward. We are unaware of any other study that has
managed to produce such a fine-granularity introspection on how shared
cache space contention develops over time for co-running applications
on a real platform. For instance, this type of analysis opens new
avenues where application progress can be related to cache occupancy
requirements and scheduling priorities are adjusted accordingly. The
same can be said for the study in Section~\ref{sec:ev_wss}. To further
demonstrate that \cachedump enables new types of cache analysis
previously impossible on real hardware, we have used the additional
space available to us to add Section~\ref{sec:ev_compat}
and~\ref{sec:ev_repl}.

\item {\bf\emph{The reviewer compares the utility of this approach to
    simulators and maintains that simulators can be used to arrive at
    the same results as those in the paper, minus the overhead.}}

  While simulators can also accomplish these goals,
  their accuracy is constrained by the model of the platform
  they simulate. Even known cycle-accurate simulators
  (e.g. Gem5) do not simulate all the moving parts of the system and
  make important approximations to generalize to a family of CPUs
  rather than a specific model. The gap between
  simulators and real platforms is palpable
  \footnote{\url{https://ieeexplore.ieee.org/abstract/document/6322869}}. Moreover,
  simulation of a full-system setup and with realistic applications is
  very inefficient and time-consuming. Lastly, even a \emph{good}
  simulator such as Gem5 can be inaccurate enough to result in some
  benchmarks not executing correctly in
  simulation\footnote{\url{https://gem5art.readthedocs.io/en/latest/tutorials/spec2017-tutorial.html}
  }. Similar shortcomings are also shared by (dynamic) binary
  instrumentation tools such as Valgrind --- see the limitations of
  CacheGrind\footnote{See Section 5.8.3 at
    \url{https://valgrind.org/docs/manual/cg-manual.html}}.

  We do not, however, envision \cachedump 
  competing with simulators. We hope \cachedump
  can (1) supplement models used to more accurately simulate real
  platforms, strengthening, or correcting them; and (2) provide more
  accurate information than traditional simulation models by
  considering realistic full-system setups --- i.e., with realistic
  file-systems, background services, network activity and so on.



%%%  RM: rephrased above.
%% the variance--introduced by the interplay of processes--in a real
%% system severely impedes their utility.  For instance, a full list of
%% the \textit{many} shortcomings of Valgrind’s cache profiler can be
%% found at https://valgrind.org/docs/manual/cg-manual.html Our tool, in
%% contrast, addresses most of these drawbacks.  Further, with other
%% simulators like Gem5, there is justifiable uncertainty about their
%% accuracy CacheFlow remedies these issues by running on a live system.
%% Additionally, CacheFlow’s reliance on RAMINDEX renders it OS-agnostic,
%% though we are unable to present a proof of concept in the time
%% remaining. In conclusion,

%% Such analysis is currently only
%% possible in simulation.

\item {\bf\emph{Since the cache mapping the ARM processors studied in
    this paper are based on simple static mapping, it is questionable
    whether CacheFlow can work with other CPU/cache architectures.}}
  
  \cachedump's applicability hinges on
  a \ramindex-like interface, not on the type of
  mapping scheme employed by the cache.
  In a hypothetical platform with permutation-based mapping and
  a \ramindex interface, \cachedump can be used to
  reverse-engineer the exact rule of the
  mapping. This can be done by initializing and fetching a memory
  buffer with a known data pattern (e.g. data = physical address). One
  can then analyze the snapshots to find out at which set/way
  coordinate a given physical address was found. As we remark in
  Table~\ref{tab:hw_support}, \ramindex will be supported in ARM
  processors for the foreseeable future.

\item {\bf\emph{The execution of CacheFlow affects the I-cache.  Will
    that be a problem?}}

  No, since the I-cache is an L1 private cache. While \cachedump
  currently focuses on the LLC, in instances where one seeks to study
  the L1 cache, they can dispatch \cachedump to run on a different
  core, thus eliminating the possibility of \cachedump polluting the
  private L1 cache of the core under analysis.

\item {\bf\emph{It seems that the method for P2L reverse address
    mapping is based on that all page structures are stored in a
    physically linear array and a page structure in this array can be
    indexed by its frame number. Is this true in Linux kernels for
    other platform/architectures?}}

  We do not make such an assumption. The Linux kernel routinely
  performs physical address to page descriptor translation (and
  vice-versa). Since at least v2.6, the 
  \texttt{phys\_to\_page} macro enables this
  conversion\footnote{See
    \url{https://elixir.bootlin.com/linux/latest/ident/phys\_to\_page}
    for further information.}. We have clarified this important point
  in Section~\ref{sec:impl_dumper}.

\item {\bf\emph{The differences between sync and async mode, and their
    use cases are unclear.}}

  Section~\ref{sec:sync_vs_async_mode} now expounds
  the workings of both modes. At a high level, synchronous mode
  facilitates more precise analysis of applications executing in
  parallel on multiple cores.  The \trigger pauses execution of
  observed applications via SIGSTOP signals, acquires a cache
  snapshot, and then resumes execution.  Asynchronous mode removes the
  coordination between the \trigger and observed applications via
  POSIX signals. It can be used in instances where only one
  application is running/being studied, or the analysis centers around
  the noise introduced by system services. Figure~\ref{fig:timeline}
  in the paper provides a bird's-eye view of both modes.

\item {\bf\emph{The \dumper's overall method of operation is
    unclear. What is the need to use POSIX signals when the authors
    also mention using IPIs to stop processes on other cores.}}

  Section~\ref{sec:sync_vs_async_mode} better explains the
  \dumper's operation modes. \dumper works by
  dispatching an inter-processor interrupt (IPI) to place CPUs in a
  busy-waiting loop, \textit{regardless of the mode used} i.e. \dumper
  will \textit{always} dispatch IPIs to stop processes while acquiring
  a snapshot.  This is different from sending POSIX signals to halt
  processes. Applications are paused to ensure that their progress is
  synchronized. Conversely, all the other cores are placed in a
  spinlock to ensure that no CPU modifies the content of the LLC while
  all the 32,768 cache lines are read from the \ramindex
  interface. We have clarified this further at the end of
  Section~\ref{sec:sync_vs_async_mode}.

  %% Synchronous mode, described in section
  %% \ref{sec:overview}, necessitates the use of POSIX signals to ensure
  %% fairness in computation when applications are executing on multiple
  %% cores.  This is because if an application among a set of
  %% applications running on multiple cores were to share a core with the
  %% Trigger, this application would have to wait for Trigger to finish
  %% processing, while applications on other shares would not be impeded.
  %% SIGSTOP/SIGCONT help alleviate concerns stemming from this
  %% problem. While we could eliminate the use of POSIX signals, we
  %% always have to rely on IPIs because they ensure that the snapshot
  %% being acquired is accurate and representative. If IPIs were not
  %% used, extraneous processes would continue polluting the cache, thus
  %% degrading the signal to noise ratio.

\item {\bf\emph{It is not clear why the authors proposed flushing the
    cache periodically.}}

  Flushing the cache spurred quite a few concerns. 
  To address them, we draw a distinction between 2
  modes in which CacheFlow can operate:
  \textit{flush mode} and \textit{transparent mode}.  Previously,
  transparent mode was not included because our evaluations centered
  around active-set analyses.  Now, flush mode facilitates active set
  analysis as before, while transparent mode minimizes cache
  pollution. When studying multiple applications across sequential
  runs, flush mode ensures that the cache only contains current
  content, allowing us to make informed comments about how well the
  application exploits cache resources --- see the cache reuse
  analysis added in Section~\ref{sec:ev_compat}.
  Figures~\ref{fig:synth_fl} and~\ref{fig:synth_tr} now highlight the
  difference in snapshots produced by the two modes on the same
  synthetic benchmark.
  
\end{enumerate}

\subsection{Reviewer \#2}

\begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label={\bf Q\arabic*:}]

\item {\bf\emph{The software instrumentation approach has a serious
    performance cost [...]; There will be a pretty serious limit to
    what can be realistically observed with an invasive technique.}}

  \cachedump is deliberately invasive in flush mode.  Contents of the
  cache can be almost entirely preserved in full transparent mode,
  with pollution limited to about 1\% of the cache size. Please see
  the new evaluation in Section~\ref{sec:ev_overh} and the description
  of flush vs. transparent mode in
  Section~\ref{sec:flush_vs_transparent_mode}.

\item {\bf\emph{How does it compare to an inexpensive JTAG solution?}}

  Kindly see our response to MR3. Cheap (JTAG) debuggers do
  not support cache snapshotting. Even industrial-grade debuggers are
  not necessarily compatible, despite a trace port being available on
  the
  target\footnote{\url{https://forums.developer.nvidia.com/t/tx1-som-jtag-debuggers/41031}}.
  \cachedump is freely available and works on system with CPUs that
  provide a \ramindex interface. It can also be used to analyize
  targets without a trace port --- common case in production devices
  --- or remotely deployed.

\item {\bf\emph{The results certainly match what I'd intuitively
    expect, but I have no idea whether they're precise enough to
    answer specific questions.}}

  To demonstrate that \cachedump facilitates meaningful analyses,
  we have added an experiment where cache reuse is
  computed to predict whether or not two applications scheduled in
  parallel will suffer any slowdown due to clash on cache
  resources. The experiment is detailed in
  Section~\ref{sec:ev_compat}.
\end{enumerate}

\subsection{Reviewer \#3}
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt, label={\bf Q\arabic*:}]
    
  \item {\bf\emph{My major concern about the paper is that it does not
      provide any performance overhead results; the driver program
      itself consumes a large portion of cache space, e.g., 50\%-60\%
      of the total capacity for 2ms sampling interval. How this
      affects the cache behavior of the application under analysis?}}
    
    Kindly see our response to MR2 above. The 50\%-60\% was not meant
    to be a measure of overhead. The point of
    the previous figure was to evaluate how much of the cache content
    was the synthetic benchmark able to ``touch'' between two
    snapshots acquired in flush mode. We have better clarified the
    difference between flush and transparent mode and replaced the
    experiment that spurred the confusion.
    
\end{enumerate}

%% \textbf{Q: Reviewer \#1 questions the utility and novelty of
%%   \cachedump, arguing that while . Additionally, }

%% A: We performed additional experiments to demonstrate novel
%% information we can obtain using CacheFlow. These are detailed
%% in section \ref{sec:eval} of the paper, and summarized here, for brevity.
%% First, we study and predict the contention for cache resources
%% among co-running applications in section VII-F. Second, we infer
%% the cache replacement policy and interpret its statistical
%% characteristics in section VII-G.
%% \\\\
%% \\\\

%%   Consider a scenario where 80\% of the cache lines were occupied by
%%   some application X. In a subsequent run, assume application Y,
%%   executed concurrently with X, occupies 20\% of the cache. Without
%%   flushing, it would be impossible to tell whether Y occupies 20\% of
%%   the cache because application X is competing for cache resources, or
%%   because Y only needs 20\% of the cache. Phrased differently,
%%   \textbf{it is impossible to correlate cache lines with an
%%     application’s progress, without flushing the cache between
%%     snapshots.} There are admittedly justifications for not flushing
%%   the cache and transparent mode can be used in those situations. For
%%   reuse analysis, however, flush mode remains vital.  \\ Further,
%%   figure 5 misled reviewers by hyperbolizing the cost incurred by
%%   using \cachedump. While the parent/driver program did occupy 50-60\%
%%   of the cache, it only did this because it could. The synthetic
%%   benchmark did not need to occupy too much of the cache, which meant
%%   that the rest of the cache remained available. This is evinced by
%%   the SD-VBS benchmark plots: we see that the benchmarks take up as
%%   much of the cache they need, reducing the number of L2 lines taken
%%   up by the parent program. Figure 4 reinforces the low overhead
%%   \cachedump actually imposes on the system by showing a heat map of a
%%   synthetic benchmark without flushing the cache. We see there that
%%   without flushing the cache between iterations, much of the cache
%%   state remains unencumbered by \cachedump.

%% \textbf{Reviewers question the rationale behind flushing the
%%   cache. While it may enable working set analysis, the workflow incurs
%%   a significant cost in terms of overhead (as high as 50\%-60\% in
%%   figure 5.), thus rendering \cachedump virtually unusable.}


%% \textbf{Q: Reviewers contend that this study needs to further
%% expound the overhead introduced by \cachedump.}

%% A: We have updated section \ref{sec:eval} to document the
%% overhead \cachedump introduces and summarized the 
%% results in Table II. In the \textit{full transparent} mode,
%% the mean space overhead across 100 runs for each 
%% benchmark hovers around 1.4\% while the time overhead
%% is about 190,000 CPU cycles in the same mode. This 
%% overhead marginally increases to about 7\% space
%% overhead and about 340,000 CPU cycles when either
%% the addresses or the layouts are resolved. Resolving both
%% the addresses and the layouts thus results in a space
%% overhead of about 13.4\% and a time overhead of about
%% 340,000 CPU cycles, which is acceptable for a
%% software-based solution.
%% \\\\
%% \textbf{Q: Reviewers express skepticism at authors' claims
%% about the viability of a software approach over hardware
%% debuggers, especially considering the fact that such
%% debuggers are relatively inexpensive.
%% As such, authors are encouraged to substantiate
%% \cachedump's results with those of a simple
%% JTAG debugger.}

%% 2. Hardware solutions cannot be used in the cloud (e.g. if one were
%% using a VPS, for instance), while CacheFlow can, thus making this tool
%% viable not just for its financial cost (open source and free), but
%% more importantly, for its general applicability in situations where
%% hardware debuggers are unusable.  \\\\ Further, the authors are not
%% aware of a JTAG debugger that costs less than \$100 with the same set
%% of functionalities as CacheFlow. Most JTAG debuggers’ capabilities do
%% not typically extend beyond their traditional capabilities (setting
%% breakpoints and accessing memory contents).  The logistics of
%% snapshotting a cache’s contents and then associating the cached
%% physical addresses with virtual addresses through reverse lookups, all
%% the while being deprived of OS support structures is a significant
%% undertaking that likely needs significant modifications to existing
%% JTAG debuggers. Whether a low-bandwith, low-fidelity JTAG debugger
%% could even be used to accomplish this functionality is arguably an
%% open research question \footnote{It should be noted that the debuggers
%%   mentioned above both rely on the high-bandwidth trace port by
%%   default.}.  \\Thus, given both the time and financial constraints
%% involved,we opted to conduct a predictive experiment in lieu of
%% obtaining ground-truth data via hardware debuggers.  Section
%% \ref{sec:eval_clash_prediction} proffers a way to predict the effect a
%% set of co-running applications will have on each other when competing
%% for cache resources.  These predictions were generated using profiles
%% obtained from previous runs of the application under two types of
%% analyses: active set analysis and reused set analysis. These
%% predictions are then empirically verified to corroborate the
%% profiler's results.

\label{changes}\section*{Changes}
\noindent All changes are highlighted in blue and summarized below:\\
1. Revised description of the various \cachedump modes
and their usage scenarios.\\
2. A rigorous exploration of the overhead \cachedump imposes on the system.\\
3. Four additional experiments to better understand the
novel kinds of insights \cachedump can provide.\\
4. Fixed typos.
}

